Improving Confidence Estimates for Unfamiliar Examples

Intuitively, unfamiliarity should lead to lack of confidence. In reality, current algorithms often make highly confident yet wrong predictions when faced with relevant but unfamiliar examples. A classifier we trained to recognize gender is 12 times more likely to be wrong with a 99% confident prediction if presented with a subject from a different age group than those seen during training. In this paper, we compare and evaluate several methods to improve confidence estimates for unfamiliar and familiar samples. We propose a testing methodology of splitting unfamiliar and familiar samples by attribute (age, breed, subcategory) or sampling (similar datasets collected by different people at different times). We evaluate methods including confidence calibration, ensembles, distillation, and a Bayesian model and use several metrics to analyze label, likelihood, and calibration error. While all methods reduce over-confident errors, the ensemble of calibrated models performs best overall, and T-scaling performs best among the approaches with fastest inference. Our code is available at https://github.com/lizhitwo/ConfidenceEstimates . $\color{red}{\text{Please see UPDATED ERRATA.}}$

==> figures/perftable_ImageNet_MC_test_mbha_familiar.tex <==
\begin{tabular}{@{\extracolsep{4pt}} r c c c c c c  @{} }
  \toprule
  & \multicolumn{2}{c}{NLL}
  & \multicolumn{2}{c}{E99}
  & \multicolumn{2}{c}{accuracy}
 \\ \cline{2-3} \cline{4-5} \cline{6-7} \\[-0.8em]
  & familiar & novel & familiar & novel & familiar & novel \\
\midrule
uncertainty & 0.310 & 1.123 & 0.014 & 0.095 & 0.901 & 0.713 \\
distilling & 0.310 & 0.878 & 0.012 & 0.027 & 0.892 & 0.711 \\
$T$-scaling & 0.331 & 0.760 & \textbf{0.000} & \textbf{0.000} & 0.896 & 0.709 \\ \midrule
single & 0.326 & 1.128 & 0.013 & 0.087 & 0.896 & 0.709 \\
ensemble & \textbf{0.282} & 0.881 & 0.007 & 0.037 & 0.894 & 0.723 \\
bagging calibrated ensemble & 0.345 & \textbf{0.726} & \textbf{0.000} & \textbf{0.000} & 0.894 & 0.725 \\
$\mc G$-distill (ours) & 0.291 & 0.844 & 0.011 & 0.024 & 0.898 & 0.715 \\
NCR (ours) & 0.287 & 0.868 & 0.005 & 0.042 & 0.896 & 0.709 \\
\bottomrule
\end{tabular}

==> figures/perftable_ImageNet_MC_test_mbha_familiar_simple.tex <==
\begin{tabular}{@{\extracolsep{4pt}} c @{\hspace{0\tabcolsep}} c c @{\hspace{0\tabcolsep}} c c @{\hspace{0\tabcolsep}} c  @{} }
  \toprule
  \multicolumn{2}{c}{NLL}
  & \multicolumn{2}{c}{E99}
  & \multicolumn{2}{c}{accuracy}
 \\ \cline{1-2} \cline{3-4} \cline{5-6} \\[-0.8em]
  familiar & novel & familiar & novel & familiar & novel \\
\midrule
0.310 & 1.123 & 0.014 & 0.094 & 0.901 & 0.713 \\
0.302 & 0.921 & 0.007 & 0.042 & 0.895 & 0.710 \\
0.331 & 0.760 & \textbf{0.000} & \textbf{0.000} & 0.896 & 0.709 \\ \midrule
0.326 & 1.128 & 0.013 & 0.087 & 0.896 & 0.709 \\
\textbf{0.256} & 0.930 & 0.005 & 0.045 & 0.906 & 0.724 \\
0.317 & \textbf{0.723} & \textbf{0.000} & \textbf{0.000} & 0.907 & 0.725 \\
0.279 & 0.868 & 0.007 & 0.034 & 0.904 & 0.716 \\
0.308 & 0.855 & \textbf{0.001} & 0.005 & 0.896 & 0.709 \\
\bottomrule
\end{tabular}

==> figures/perftable_LFWpSex_MC_test_fm_familiar.tex <==
\begin{tabular}{@{\extracolsep{4pt}} r c c c c c c  @{} }
  \toprule
  & \multicolumn{2}{c}{NLL}
  & \multicolumn{2}{c}{E99}
  & \multicolumn{2}{c}{accuracy}
 \\ \cline{2-3} \cline{4-5} \cline{6-7} \\[-0.8em]
  & familiar & novel & familiar & novel & familiar & novel \\
\midrule
uncertainty & 0.080 & 0.567 & 0.005 & 0.068 & 0.974 & 0.854 \\
distilling & 0.082 & 0.384 & 0.002 & 0.004 & 0.972 & 0.832 \\
$T$-scaling & 0.080 & \textbf{0.328} & 0.001 & 0.003 & 0.972 & 0.853 \\ \midrule
single & 0.083 & 0.542 & 0.005 & 0.060 & 0.972 & 0.853 \\
ensemble & \textbf{0.067} & 0.483 & 0.002 & 0.047 & 0.975 & 0.839 \\
bagging calibrated ensemble & 0.080 & \textbf{0.345} & \textbf{0.000} & 0.004 & 0.976 & 0.838 \\
$\mc G$-distill (ours) & 0.078 & 0.358 & 0.001 & \textbf{0.002} & 0.972 & 0.837 \\
NCR (ours) & 0.074 & 0.380 & 0.002 & 0.020 & 0.972 & 0.853 \\
\bottomrule
\end{tabular}

==> figures/perftable_LFWpSex_MC_test_fm_familiar_densenet161.tex <==
\begin{tabular}{@{\extracolsep{4pt}} r c c c c c c  @{} }
  \toprule
  & \multicolumn{2}{c}{NLL}
  & \multicolumn{2}{c}{E99}
  & \multicolumn{2}{c}{accuracy}
 \\ \cline{2-3} \cline{4-5} \cline{6-7} \\[-0.8em]
  & familiar & novel & familiar & novel & familiar & novel \\
\midrule
uncertainty & 0.080 & 0.593 & 0.007 & 0.074 & 0.978 & 0.858 \\
distilling & 0.068 & 0.371 & 0.002 & 0.009 & 0.977 & 0.849 \\
$T$-scaling & \textbf{0.062} & \textbf{0.328} & 0.001 & 0.008 & 0.978 & 0.857 \\ \midrule
single & 0.077 & 0.561 & 0.006 & 0.066 & 0.978 & 0.857 \\
ensemble & \textbf{0.063} & 0.428 & 0.003 & 0.033 & 0.978 & 0.846 \\
bagging calibrated ensemble & 0.066 & \textbf{0.308} & \textbf{0.000} & \textbf{0.001} & 0.978 & 0.848 \\
$\mc G$-distill (ours) & 0.067 & 0.365 & 0.002 & 0.010 & 0.978 & 0.843 \\
NCR (ours) & \textbf{0.062} & 0.374 & 0.002 & 0.020 & 0.978 & 0.857 \\
\bottomrule
\end{tabular}

==> figures/perftable_LFWpSex_MC_test_fm_familiar_simple.tex <==
\begin{tabular}{@{\extracolsep{4pt}} r c @{\hspace{0\tabcolsep}} c c @{\hspace{0\tabcolsep}} c c @{\hspace{0\tabcolsep}} c  @{} }
  \toprule
  & \multicolumn{2}{c}{NLL}
  & \multicolumn{2}{c}{E99}
  & \multicolumn{2}{c}{accuracy}
 \\ \cline{2-3} \cline{4-5} \cline{6-7} \\[-0.8em]
  & familiar & novel & familiar & novel & familiar & novel \\
\midrule
uncertainty & 0.080 & 0.567 & 0.005 & 0.068 & 0.974 & 0.853 \\
distilling & 0.077 & 0.364 & 0.001 & \textbf{0.002} & 0.973 & 0.844 \\
$T$-scaling & 0.080 & \textbf{0.328} & 0.001 & 0.003 & 0.972 & 0.853 \\ \midrule
single & 0.083 & 0.542 & 0.005 & 0.060 & 0.972 & 0.853 \\
ensemble & \textbf{0.062} & 0.455 & 0.002 & 0.039 & 0.978 & 0.853 \\
calib. ens. & 0.074 & \textbf{0.313} & \textbf{0.000} & \textbf{0.001} & 0.979 & 0.852 \\
$\mc G$-distill (ours) & 0.073 & 0.337 & 0.001 & \textbf{0.001} & 0.975 & 0.847 \\
NCR (ours) & 0.089 & 0.334 & 0.001 & \textbf{0.001} & 0.972 & 0.854 \\
\bottomrule
\end{tabular}

==> figures/perftable_LFWpSex_MC_test_fm_familiar_simple_densenet161.tex <==
\begin{tabular}{@{\extracolsep{4pt}} r c c c c c c  @{} }
  \toprule
  & \multicolumn{2}{c}{NLL}
  & \multicolumn{2}{c}{E99}
  & \multicolumn{2}{c}{accuracy}
 \\ \cline{2-3} \cline{4-5} \cline{6-7} \\[-0.8em]
  & familiar & novel & familiar & novel & familiar & novel \\
\midrule
uncertainty & 0.080 & 0.593 & 0.007 & 0.074 & 0.978 & 0.859 \\
distilling & 0.071 & 0.412 & 0.004 & 0.025 & 0.979 & 0.865 \\
$T$-scaling & 0.062 & 0.328 & 0.001 & 0.008 & 0.978 & 0.857 \\ \midrule
single & 0.077 & 0.561 & 0.006 & 0.066 & 0.978 & 0.857 \\
ensemble & \textbf{0.051} & 0.410 & 0.002 & 0.035 & 0.982 & 0.866 \\
calib. ens. & 0.053 & \textbf{0.284} & \textbf{0.000} & \textbf{0.001} & 0.982 & 0.866 \\
$\mc G$-distill (ours) & 0.064 & 0.356 & 0.003 & 0.014 & 0.980 & 0.861 \\
NCR (ours) & 0.082 & 0.323 & 0.001 & \textbf{0.000} & 0.978 & 0.859 \\
\bottomrule
\end{tabular}

==> figures/perftable_OIIITPets_MC_test_catvdog_familiar.tex <==
\begin{tabular}{@{\extracolsep{4pt}} r c c c c c c  @{} }
  \toprule
  & \multicolumn{2}{c}{NLL}
  & \multicolumn{2}{c}{E99}
  & \multicolumn{2}{c}{accuracy}
 \\ \cline{2-3} \cline{4-5} \cline{6-7} \\[-0.8em]
  & familiar & novel & familiar & novel & familiar & novel \\
\midrule
0.056 & 0.417 & 0.004 & 0.053 & 0.985 & 0.907 \\
0.069 & 0.362 & 0.001 & 0.039 & 0.979 & 0.888 \\
\textbf{0.040} & 0.275 & 0.001 & 0.017 & 0.984 & 0.905 \\ \midrule
0.053 & 0.423 & 0.004 & 0.053 & 0.984 & 0.905 \\
0.046 & 0.292 & 0.001 & 0.023 & 0.982 & 0.901 \\
0.046 & \textbf{0.233} & \textbf{0.000} & \textbf{0.004} & 0.982 & 0.904 \\
0.071 & 0.311 & 0.002 & 0.022 & 0.978 & 0.893 \\
\textbf{0.041} & 0.304 & 0.001 & 0.025 & 0.984 & 0.905 \\
\bottomrule
\end{tabular}

==> figures/perftable_OIIITPets_MC_test_catvdog_familiar_simple.tex <==
\begin{tabular}{@{\extracolsep{4pt}} c @{\hspace{0\tabcolsep}} c c @{\hspace{0\tabcolsep}} c c @{\hspace{0\tabcolsep}} c  @{} }
  \toprule
  \multicolumn{2}{c}{NLL}
  & \multicolumn{2}{c}{E99}
  & \multicolumn{2}{c}{accuracy}
 \\ \cline{1-2} \cline{3-4} \cline{5-6} \\[-0.8em]
  familiar & novel & familiar & novel & familiar & novel \\
\midrule
0.056 & 0.417 & 0.004 & 0.053 & 0.984 & 0.908 \\
0.060 & 0.332 & 0.002 & 0.036 & 0.982 & 0.901 \\
0.040 & 0.275 & 0.001 & 0.017 & 0.984 & 0.905 \\ \midrule
0.053 & 0.423 & 0.004 & 0.053 & 0.984 & 0.905 \\
\textbf{0.033} & 0.286 & 0.001 & 0.024 & 0.988 & 0.912 \\
\textbf{0.032} & \textbf{0.220} & \textbf{0.000} & 0.010 & 0.988 & 0.912 \\
0.062 & 0.307 & 0.001 & 0.022 & 0.979 & 0.897 \\
0.063 & 0.288 & \textbf{0.000} & \textbf{0.000} & 0.984 & 0.904 \\
\bottomrule
\end{tabular}

==> figures/perftable_VOC2COCO_ML_test_20cls_familiar.tex <==
\begin{tabular}{@{\extracolsep{4pt}} r c c c c c c  @{} }
  \toprule
  & \multicolumn{2}{c}{NLL}
  & \multicolumn{2}{c}{E99}
  & \multicolumn{2}{c}{mAP}
 \\ \cline{2-3} \cline{4-5} \cline{6-7} \\[-0.8em]
  & familiar & novel & familiar & novel & familiar & novel \\
\midrule
uncertainty & 0.086 & 0.129 & 0.003 & 0.006 & 0.806 & 0.543 \\
distilling & 0.088 & \textbf{0.122} & 0.001 & 0.004 & 0.805 & 0.542 \\
$T$-scaling & 0.087 & 0.127 & 0.001 & 0.003 & 0.805 & 0.545 \\ \midrule
single & 0.086 & 0.128 & 0.002 & 0.005 & 0.805 & 0.545 \\
ensemble & \textbf{0.084} & 0.124 & 0.002 & 0.005 & 0.810 & 0.552 \\
bagging calibrated ensemble & 0.086 & 0.124 & \textbf{0.001} & \textbf{0.003} & 0.810 & 0.552 \\
$\mc G$-distill (ours) & 0.088 & \textbf{0.123} & 0.001 & 0.004 & 0.798 & 0.538 \\
NCR (ours) & 0.096 & 0.144 & 0.001 & 0.004 & 0.804 & 0.539 \\
\bottomrule
\end{tabular}

==> figures/perftable_VOC2COCO_ML_test_20cls_familiar_simple.tex <==
\begin{tabular}{@{\extracolsep{4pt}} r c @{\hspace{0\tabcolsep}} c c @{\hspace{0\tabcolsep}} c c @{\hspace{0\tabcolsep}} c  @{} }
  \toprule
  & \multicolumn{2}{c}{NLL}
  & \multicolumn{2}{c}{E99}
  & \multicolumn{2}{c}{mAP}
 \\ \cline{2-3} \cline{4-5} \cline{6-7} \\[-0.8em]
  & familiar & novel & familiar & novel & familiar & novel \\
\midrule
uncertainty & 0.086 & 0.129 & 0.003 & 0.006 & 0.806 & 0.543 \\
distilling & 0.087 & \textbf{0.122} & 0.001 & 0.003 & 0.807 & 0.547 \\
$T$-scaling & 0.087 & 0.127 & 0.001 & 0.003 & 0.805 & 0.545 \\ \midrule
single & 0.086 & 0.128 & 0.002 & 0.005 & 0.805 & 0.545 \\
ensemble & \textbf{0.082} & 0.123 & 0.002 & 0.005 & 0.817 & 0.559 \\
calib. ens. & 0.084 & 0.123 & \textbf{0.001} & \textbf{0.003} & 0.817 & 0.559 \\
$\mc G$-distill (ours) & 0.087 & 0.122 & 0.001 & 0.003 & 0.802 & 0.541 \\
NCR (ours) & 0.087 & 0.125 & 0.002 & 0.004 & 0.804 & 0.544 \\
\bottomrule
\end{tabular}

==> figures/perftable_diffens_ImageNet_MC_test_mbha_familiar.tex <==
\begin{tabular}{@{\extracolsep{4pt}} r c c c c c c  @{} }
  \toprule
  & \multicolumn{2}{c}{NLL}
  & \multicolumn{2}{c}{E99}
  & \multicolumn{2}{c}{accuracy}
 \\ \cline{2-3} \cline{4-5} \cline{6-7} \\[-0.8em]
  & familiar & novel & familiar & novel & familiar & novel \\
\midrule
simple distilling & 0.302 & 0.921 & 0.007 & 0.042 & 0.895 & 0.710 \\
simple ensemble & \textbf{0.256} & 0.930 & \textbf{0.005} & 0.045 & 0.906 & 0.724 \\
simple $\mc G$-distill & 0.279 & 0.868 & \textbf{0.007} & 0.034 & 0.904 & 0.716 \\ \midrule
bagging distilling & 0.310 & 0.878 & 0.012 & \textbf{0.027} & 0.892 & 0.711 \\
bagging ensemble & 0.282 & 0.881 & 0.007 & 0.037 & 0.894 & 0.723 \\
bagging $\mc G$-distill & 0.291 & \textbf{0.844} & 0.011 & \textbf{0.024} & 0.898 & 0.715 \\
\bottomrule
\end{tabular}

==> figures_x10/perftable_ImageNet_MC_test_mbha_familiar.tex <==
\begin{tabular}{@{\extracolsep{4pt}} r c c c c c c  @{} }
  \toprule
  & \multicolumn{2}{c}{NLL}
  & \multicolumn{2}{c}{E99}
  & \multicolumn{2}{c}{accuracy}
 \\ \cline{2-3} \cline{4-5} \cline{6-7} \\[-0.8em]
  & familiar & novel & familiar & novel & familiar & novel \\
\midrule
uncertainty & 0.310 & 1.123 & 0.014 & 0.094 & 0.900 & 0.713 \\
distilling & 0.310 & 0.878 & 0.012 & 0.027 & 0.892 & 0.711 \\ \midrule
single & 0.326 & 1.128 & 0.013 & 0.087 & 0.896 & 0.709 \\
ensemble & \textbf{0.282} & 0.881 & \textbf{0.007} & 0.037 & 0.894 & 0.723 \\
$\mc G$-distill (ours) & 0.291 & 0.844 & 0.011 & 0.024 & 0.898 & 0.715 \\
distilling $\times 10$ & 0.292 & 0.828 & 0.012 & \textbf{0.019} & 0.899 & 0.723 \\
$\mc G$-distill $\times 10$ & \textbf{0.279} & \textbf{0.810} & 0.012 & 0.023 & 0.901 & 0.719 \\
\bottomrule
\end{tabular}

==> figures_x10/perftable_ImageNet_MC_test_mbha_familiar_simple.tex <==
\begin{tabular}{@{\extracolsep{4pt}} r c c c c c c  @{} }
  \toprule
  & \multicolumn{2}{c}{NLL}
  & \multicolumn{2}{c}{E99}
  & \multicolumn{2}{c}{accuracy}
 \\ \cline{2-3} \cline{4-5} \cline{6-7} \\[-0.8em]
  & familiar & novel & familiar & novel & familiar & novel \\
\midrule
uncertainty & 0.310 & 1.122 & 0.014 & 0.094 & 0.900 & 0.714 \\
distilling & 0.302 & 0.921 & 0.007 & 0.042 & 0.895 & 0.710 \\
single & 0.326 & 1.128 & 0.013 & 0.087 & 0.896 & 0.709 \\ \midrule
ensemble & \textbf{0.256} & 0.930 & 0.005 & 0.045 & 0.906 & 0.724 \\
calib. ens. & 0.317 & \textbf{0.723} & \textbf{0.000} & \textbf{0.000} & 0.907 & 0.725 \\
$\mc G$-distill (ours) & 0.279 & 0.868 & 0.007 & 0.034 & 0.904 & 0.716 \\
distilling $\times 10$ & 0.275 & 0.846 & 0.005 & 0.030 & 0.903 & 0.720 \\
$\mc G$-distill $\times 10$ & 0.263 & 0.819 & 0.005 & 0.026 & 0.915 & 0.719 \\
\bottomrule
\end{tabular}

==> figures_x10/perftable_LFWpSex_MC_test_fm_familiar.tex <==
\begin{tabular}{@{\extracolsep{4pt}} r c c c c c c  @{} }
  \toprule
  & \multicolumn{2}{c}{NLL}
  & \multicolumn{2}{c}{E99}
  & \multicolumn{2}{c}{accuracy}
 \\ \cline{2-3} \cline{4-5} \cline{6-7} \\[-0.8em]
  & familiar & novel & familiar & novel & familiar & novel \\
\midrule
uncertainty & 0.080 & 0.567 & 0.005 & 0.068 & 0.974 & 0.853 \\
distilling & 0.082 & 0.384 & 0.002 & 0.004 & 0.972 & 0.832 \\ \midrule
single & 0.083 & 0.542 & 0.005 & 0.060 & 0.972 & 0.853 \\
ensemble & \textbf{0.067} & 0.483 & 0.002 & 0.047 & 0.975 & 0.839 \\
$\mc G$-distill (ours) & 0.078 & \textbf{0.358} & 0.001 & \textbf{0.002} & 0.972 & 0.837 \\
distilling $\times 10$ & 0.077 & 0.363 & \textbf{0.001} & \textbf{0.001} & 0.973 & 0.835 \\
$\mc G$-distill $\times 10$ & 0.074 & \textbf{0.341} & \textbf{0.001} & \textbf{0.001} & 0.976 & 0.841 \\
\bottomrule
\end{tabular}

==> figures_x10/perftable_LFWpSex_MC_test_fm_familiar_densenet161.tex <==
\begin{tabular}{@{\extracolsep{4pt}} r c c c c c c  @{} }
  \toprule
  & \multicolumn{2}{c}{NLL}
  & \multicolumn{2}{c}{E99}
  & \multicolumn{2}{c}{accuracy}
 \\ \cline{2-3} \cline{4-5} \cline{6-7} \\[-0.8em]
  & familiar & novel & familiar & novel & familiar & novel \\
\midrule
uncertainty & 0.080 & 0.593 & 0.007 & 0.074 & 0.978 & 0.858 \\
distilling & 0.068 & 0.371 & 0.002 & 0.009 & 0.977 & 0.849 \\ \midrule
single & 0.077 & 0.561 & 0.006 & 0.066 & 0.978 & 0.857 \\
ensemble & 0.063 & 0.428 & 0.003 & 0.033 & 0.978 & 0.846 \\
$\mc G$-distill (ours) & 0.067 & 0.365 & 0.002 & 0.010 & 0.978 & 0.843 \\
distilling $\times 10$ & \textbf{0.059} & \textbf{0.331} & \textbf{0.001} & \textbf{0.003} & 0.980 & 0.846 \\
$\mc G$-distill $\times 10$ & \textbf{0.059} & \textbf{0.335} & 0.001 & 0.005 & 0.980 & 0.845 \\
\bottomrule
\end{tabular}

==> figures_x10/perftable_LFWpSex_MC_test_fm_familiar_simple.tex <==
\begin{tabular}{@{\extracolsep{4pt}} r c c c c c c  @{} }
  \toprule
  & \multicolumn{2}{c}{NLL}
  & \multicolumn{2}{c}{E99}
  & \multicolumn{2}{c}{accuracy}
 \\ \cline{2-3} \cline{4-5} \cline{6-7} \\[-0.8em]
  & familiar & novel & familiar & novel & familiar & novel \\
\midrule
uncertainty & 0.080 & 0.567 & 0.005 & 0.068 & 0.974 & 0.853 \\
distilling & 0.077 & 0.364 & 0.001 & 0.002 & 0.973 & 0.844 \\
single & 0.083 & 0.542 & 0.005 & 0.060 & 0.972 & 0.853 \\ \midrule
ensemble & \textbf{0.062} & 0.455 & 0.002 & 0.039 & 0.978 & 0.853 \\
calib. ens. & 0.074 & \textbf{0.313} & \textbf{0.000} & 0.001 & 0.979 & 0.852 \\
$\mc G$-distill (ours) & 0.073 & 0.337 & 0.001 & 0.001 & 0.975 & 0.847 \\
distilling $\times 10$ & 0.071 & 0.339 & 0.001 & 0.001 & 0.978 & 0.847 \\
$\mc G$-distill $\times 10$ & 0.068 & 0.320 & 0.001 & \textbf{0.000} & 0.980 & 0.850 \\
\bottomrule
\end{tabular}

==> figures_x10/perftable_LFWpSex_MC_test_fm_familiar_simple_densenet161.tex <==
\begin{tabular}{@{\extracolsep{4pt}} r c c c c c c  @{} }
  \toprule
  & \multicolumn{2}{c}{NLL}
  & \multicolumn{2}{c}{E99}
  & \multicolumn{2}{c}{accuracy}
 \\ \cline{2-3} \cline{4-5} \cline{6-7} \\[-0.8em]
  & familiar & novel & familiar & novel & familiar & novel \\
\midrule
uncertainty & 0.080 & 0.593 & 0.007 & 0.074 & 0.978 & 0.859 \\
distilling & 0.071 & 0.412 & 0.004 & 0.025 & 0.979 & 0.865 \\
single & 0.077 & 0.561 & 0.006 & 0.066 & 0.978 & 0.857 \\ \midrule
ensemble & \textbf{0.051} & 0.410 & 0.002 & 0.035 & 0.982 & 0.866 \\
calib. ens. & 0.053 & \textbf{0.284} & \textbf{0.000} & \textbf{0.001} & 0.982 & 0.866 \\
$\mc G$-distill (ours) & 0.064 & 0.356 & 0.003 & 0.014 & 0.980 & 0.861 \\
distilling $\times 10$ & 0.053 & 0.336 & 0.002 & 0.008 & 0.983 & 0.868 \\
$\mc G$-distill $\times 10$ & 0.053 & 0.313 & 0.002 & 0.005 & 0.982 & 0.861 \\
\bottomrule
\end{tabular}

==> figures_x10/perftable_OIIITPets_MC_test_catvdog_familiar.tex <==
\begin{tabular}{@{\extracolsep{4pt}} r c c c c c c  @{} }
  \toprule
  & \multicolumn{2}{c}{NLL}
  & \multicolumn{2}{c}{E99}
  & \multicolumn{2}{c}{accuracy}
 \\ \cline{2-3} \cline{4-5} \cline{6-7} \\[-0.8em]
  & familiar & novel & familiar & novel & familiar & novel \\
\midrule
uncertainty & 0.056 & 0.418 & 0.005 & 0.054 & 0.984 & 0.908 \\
distilling & 0.069 & 0.362 & 0.001 & 0.039 & 0.979 & 0.888 \\ \midrule
single & 0.053 & 0.423 & 0.004 & 0.053 & 0.984 & 0.905 \\
ensemble & \textbf{0.046} & 0.292 & 0.001 & 0.023 & 0.982 & 0.901 \\
$\mc G$-distill (ours) & 0.071 & 0.311 & 0.002 & 0.022 & 0.978 & 0.893 \\
distilling $\times 10$ & 0.060 & 0.305 & \textbf{0.000} & 0.017 & 0.980 & 0.893 \\
$\mc G$-distill $\times 10$ & 0.063 & \textbf{0.262} & \textbf{0.000} & \textbf{0.004} & 0.981 & 0.892 \\
\bottomrule
\end{tabular}

==> figures_x10/perftable_OIIITPets_MC_test_catvdog_familiar_simple.tex <==
\begin{tabular}{@{\extracolsep{4pt}} r c c c c c c  @{} }
  \toprule
  & \multicolumn{2}{c}{NLL}
  & \multicolumn{2}{c}{E99}
  & \multicolumn{2}{c}{accuracy}
 \\ \cline{2-3} \cline{4-5} \cline{6-7} \\[-0.8em]
  & familiar & novel & familiar & novel & familiar & novel \\
\midrule
uncertainty & 0.055 & 0.417 & 0.005 & 0.053 & 0.984 & 0.907 \\
distilling & 0.060 & 0.332 & 0.002 & 0.036 & 0.982 & 0.901 \\
single & 0.053 & 0.423 & 0.004 & 0.053 & 0.984 & 0.905 \\ \midrule
ensemble & \textbf{0.033} & 0.286 & 0.001 & 0.024 & 0.988 & 0.912 \\
calib. ens. & \textbf{0.032} & \textbf{0.220} & \textbf{0.000} & 0.010 & 0.988 & 0.912 \\
$\mc G$-distill (ours) & 0.062 & 0.307 & 0.001 & 0.022 & 0.979 & 0.897 \\
distilling $\times 10$ & 0.047 & 0.259 & 0.001 & 0.010 & 0.985 & 0.910 \\
$\mc G$-distill $\times 10$ & 0.050 & 0.245 & \textbf{0.000} & \textbf{0.003} & 0.984 & 0.902 \\
\bottomrule
\end{tabular}

==> figures_x10/perftable_VOC2COCO_ML_test_20cls_familiar.tex <==
\begin{tabular}{@{\extracolsep{4pt}} r c c c c c c  @{} }
  \toprule
  & \multicolumn{2}{c}{NLL}
  & \multicolumn{2}{c}{E99}
  & \multicolumn{2}{c}{mAP}
 \\ \cline{2-3} \cline{4-5} \cline{6-7} \\[-0.8em]
  & familiar & novel & familiar & novel & familiar & novel \\
\midrule
uncertainty & 0.086 & 0.129 & 0.003 & 0.006 & 0.806 & 0.543 \\
distilling & 0.088 & 0.122 & 0.001 & 0.004 & 0.805 & 0.542 \\ \midrule
single & 0.086 & 0.128 & 0.002 & 0.005 & 0.805 & 0.545 \\
ensemble & \textbf{0.084} & 0.124 & 0.002 & 0.005 & 0.810 & 0.552 \\
$\mc G$-distill (ours) & 0.088 & 0.123 & 0.001 & 0.004 & 0.798 & 0.538 \\
distilling $\times 10$ & 0.086 & \textbf{0.121} & \textbf{0.001} & \textbf{0.003} & 0.811 & 0.550 \\
$\mc G$-distill $\times 10$ & 0.087 & 0.121 & 0.001 & 0.003 & 0.803 & 0.544 \\
\bottomrule
\end{tabular}

==> figures_x10/perftable_VOC2COCO_ML_test_20cls_familiar_simple.tex <==
\begin{tabular}{@{\extracolsep{4pt}} r c c c c c c  @{} }
  \toprule
  & \multicolumn{2}{c}{NLL}
  & \multicolumn{2}{c}{E99}
  & \multicolumn{2}{c}{mAP}
 \\ \cline{2-3} \cline{4-5} \cline{6-7} \\[-0.8em]
  & familiar & novel & familiar & novel & familiar & novel \\
\midrule
uncertainty & 0.086 & 0.129 & 0.003 & 0.006 & 0.806 & 0.543 \\
distilling & 0.087 & 0.122 & 0.001 & 0.003 & 0.807 & 0.547 \\
single & 0.086 & 0.128 & 0.002 & 0.005 & 0.805 & 0.545 \\ \midrule
ensemble & \textbf{0.082} & 0.123 & 0.002 & 0.005 & 0.817 & 0.559 \\
calib. ens. & 0.084 & 0.123 & \textbf{0.001} & \textbf{0.003} & 0.817 & 0.559 \\
$\mc G$-distill (ours) & 0.087 & 0.122 & 0.001 & 0.003 & 0.802 & 0.541 \\
distilling $\times 10$ & 0.085 & \textbf{0.120} & 0.001 & 0.003 & 0.813 & 0.555 \\
$\mc G$-distill $\times 10$ & 0.086 & 0.121 & 0.001 & 0.003 & 0.807 & 0.547 \\
\bottomrule
\end{tabular}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
